LightSecAgg: a Lightweight and Versatile Design for Secure Aggregation in Federated Learning

Secure model aggregation is a key component of federated learning (FL) that aims at protecting the privacy of each user's individual model while allowing for their global aggregation. It can be applied to any aggregation-based FL approach for training a global or personalized model. Model aggregation needs to also be resilient against likely user dropouts in FL systems, making its design substantially more complex. State-of-the-art secure aggregation protocols rely on secret sharing of the random-seeds used for mask generations at the users to enable the reconstruction and cancellation of those belonging to the dropped users. The complexity of such approaches, however, grows substantially with the number of dropped users. We propose a new approach, named LightSecAgg, to overcome this bottleneck by changing the design from "random-seed reconstruction of the dropped users" to "one-shot aggregate-mask reconstruction of the active users via mask encoding/decoding". We show that LightSecAgg achieves the same privacy and dropout-resiliency guarantees as the state-of-the-art protocols while significantly reducing the overhead for resiliency against dropped users. We also demonstrate that, unlike existing schemes, LightSecAgg can be applied to secure aggregation in the asynchronous FL setting. Furthermore, we provide a modular system design and optimized on-device parallelization for scalable implementation, by enabling computational overlapping between model training and on-device encoding, as well as improving the speed of concurrent receiving and sending of chunked masks. We evaluate LightSecAgg via extensive experiments for training diverse models on various datasets in a realistic FL system with large number of users and demonstrate that LightSecAgg significantly reduces the total training time.

==> MLSys/7-Async.tex <==
In the previous sections, we considered secure model aggregation  in the synchronous FL setting where all users train local models based on the global model with the same time stamp and the server performs a synchronized aggregation of the local models to update the global model for the next round. Synchronous FL, however, can be slow and costly for implementation across a large number of users because of the stragglers. 

Asynchronous FL tackles this challenge by incorporating the updates of the users as soon as they arrive at the server \cite{xie2019asynchronous,van2020asynchronous,chai2020fedat,chen2020asynchronous}.
While asynchronous FL handles stragglers efficiently, it introduces another challenge: staleness of the local updates.
As the server updates the global model at any time without synchronization and the users have heterogeneous conditions, this results in a mismatch in staleness between the users.
Conventional secure aggregation protocols, \google and \googlep, are not compatible with asynchronous FL protocols as the cancellation of the pairwise random masks based on the key agreement protocol is not guaranteed due to the mismatch in staleness.
% Asynchronous FL tackles the straggler problem by incorporating the updates of the users as soon as they arrive at the server \cite{xie2019asynchronous,van2020asynchronous,chai2020fedat,chen2020asynchronous}.
% While asynchronous FL handles stragglers efficiently, it introduces another challenge, staleness of the local updates.
% As the server updates the global model at any time without synchronization and the users have heterogeneous conditions, there is mismatch in staleness between the users.
% Conventional secure aggregation protocols, \google and \googlep, are not compatible with asynchronous FL protocols because the cancellation of the pairwise random masks based on the key agreement protocol is not guaranteed due to the mismatch in staleness between the users.
% While asynchronous FL handles stragglers efficiently, it is not compatible with the prior secure aggregation protocols because these protocols require many local models to be aggregated together while each single local model updates the global model in asynchronous FL.
% In asynchronous FL, each user locally trains the model and sends the local updates to the server whenever 

Unlike our baseline secure aggregation protocols, \scheme enables secure aggregation also in the asynchronous FL setting. 
We demonstrate this by describing how \scheme can be applied to asynchronous FL in the context of a recently proposed asynchronous FL protocol, \FedBuff, where the server stores each local update in a TEE-enabled \emph{secure} buffer of size $K$ and updates the global model by aggregating the stored updates when the buffer is full \cite{nguyen2021federated}.
% In contrast, \scheme can be generalized to secure aggregation in the asynchronous FL setting. 
% In contrast, \scheme enables secure aggregation also in the asynchronous FL setting. 
% To do so, here we incorporate \scheme with a recently proposed asynchronous FL protocol, \FedBuff, where the server stores each local update in a buffer of size $K$ and updates the global model by aggregating the stored updates when the buffer is full \cite{nguyen2021federated}.
% Conventional secure aggregation protocols, \google and \googlep, are not compatible with asynchronous FL protocols because the cancellation of the pairwise random masks based on the key agreement protocol is not guaranteed due to the mismatch in staleness between the users.
% On the other hand, 
The reliance of \FedBuff on TEEs limits the buffer size in this approach as TEEs have limited memory. Interestingly, \scheme can be applied to this protocol \emph{without relying on a secure buffer} by encoding the local masks in a way that the server can recover the aggregate of masks from the encoded masks via a one-shot computation, even though the masks are generated in different training rounds.
To our best knowledge, in asynchronous FL, \scheme is the first work that protects the privacy of individual models in an information-theoretic sense, i.e., without relying on differential privacy (DP) or trusted execution environments (TEEs).
The details of the \scheme protocol for asynchronous FL are presented in Appendix \ref{appendix:asyncFL}, which includes: (1) detailed description of the protocol in the asynchronous regime; (2) its theoretical guarantees; and (3) performance evaluation.

% \scheme can also be generalized to the secure aggregation in the asynchronous FL.
% For instance, we can leverage the idea of \scheme to a recently proposed asynchronous FL protocol, named \FedBuff, where the server stores each local update in a buffer of size $K$ and updates the global model by aggregating the stored updates when the buffer is full \cite{nguyen2021federated}.
% Conventional secure aggregation protocols, \google and \googlep, are not compatible with this asynchronous FL because the cancellation of the pairwise random masks based on the key agreement protocol is not guaranteed due to the mismatch in staleness between users.
% On the other hand, \scheme can be applied to this protocol by encoding the local masks in a way that the server can recover the aggregate of masks from the encoded masks via a one-shot computation even though the masks are generated in different training rounds.
% To our best knowledge, in the asynchronous FL, it is the first work to protect the privacy of individual model in information-theoretic sense, i.e., without relying on differential privacy (DP) or trusted execution environments (TEEs).
% The detail of the generalized \scheme protocol in the asynchronous FL is presented in the Appendix \ref{appendix:asyncFL}.

% Recently, a buffered asynchronous FL protocol, named \FedBuff, has been proposed which bridges the gap between synchronous and asynchronous training to mitigate the stragglers and to also ensure privacy simultaneously \cite{nguyen2021federated}. \FedBuff, however, requires a trusted execution environment (TEE) enabled private buffer.
% As the TEE has limited memory and hence cannot scale to the large size, our goal is to design a secure aggregation protocol for the asynchronous FL which enable the server to aggregate the local models in the buffer while protecting the individual local updates without relying on the TEE. 
% 
% Conventional secure aggregation protocols, \google and \googlep, are not compatible with the buffered asynchronous FL. This is because the cancellation of the pairwise random masks based on the key agreement protocol is not guaranteed due to the mismatch in staleness between users.
% On the other hand, \scheme can be generalized to the asynchronous secure aggregation.
% Our key intuition is to encode the local masks in a way that the server can recover the aggregate of masks from the encoded masks via a one-shot computation even though the masks are generated in different training rounds.
% In the Appendix \ref{appendix:asyncFL}, we present the overview of the asynchronous FL, the incompatibility of \google and \googlep with the  asynchronous FL, and the generalized \scheme protocol in asynchronous FL.
% The detail of the generalized \scheme protocol in asynchronous FL is presented in the Appendix \ref{appendix:asyncFL}.

% In this section, we provide a brief overview of \FedBuff \cite{nguyen2021federated}. Then, we illustrate the incompatibility of the conventional secure aggregation with asynchronous FL in Section \ref{subsec:incompatibility}. 
% Finally, in Section \ref{subsec:proposed-async}, we generalize \scheme to the buffered asynchronous FL setting which can protect the privacy of individual updates without relying on TEE. 

% \subsection{Overview of \FedBuff}\label{subsec:fedbuff}

% In the buffered asynchronous setting, the server stores each local model that it receives in a buffer of size $K$ and updates the global model when the buffer is full. 
% The key intuition of \FedBuff is to introduce a new design parameter $K$, the buffer size at the server, so that \FedBuff has two degrees of freedom, $K$ and the concurrency $C$  while the synchronous FL frameworks have only one degree of freedom, concurrency.
% We describe the details of \FedBuff in the Appendix \ref{app:sub:fedbuff}.

% At round $t$, user $i$ locally trains the model and sends the difference between the downloaded global model and updated model to the server, denoted by ${\Delta}^{(t;t_i)}_i$, where $t_i$ is the latest round index when the global model is downloaded by user $i$ and $t$ is the round index when the local update is sent to the server. 
% The server stores the received local updates in a buffer of size $K$. When the buffer is full, the server updates the global model by subtracting the aggregate of all local updates from the current global model.
% Thus, the goal of secure aggregation protocol in the buffered asynchronous FL is to enable the server to compute $\sum_{i\in \mathcal{S}^{(t)}} {\Delta}^{(t;t_i)}_i$ while the server cannot learn the individual local updates, ${\Delta}^{(t;t_i)}_i$ for all $i\in\mathcal{S}^{(t)}$. 
% $\mathcal{S}^{(t)}$ is an index set of the $K$ users whose local models are in the buffer at round $t$.


% \subsection{Incompatibility of \google and \googlep with Buffered Asynchronous FL}
% \label{subsec:incompatibility}

% As described in Section~\ref{sec:overviews}, \google \cite{bonawitz2017practical} and \googlep~\cite{bell2020secure} are designed for synchronous FL. At round $t$, each pair of users $i,j\in[N]$ agree on a pairwise random-seed $a_{i,j}^{(t)}$, and generate a random vector by running PRG based on the random seed of $a_{i,j}^{(t)}$ to mask the local update. 
% This additive structure has the unique property that these pairwise random vectors cancel out when the server aggregates the masked models because user $i(<j)$ adds $\mathrm{PRG}(a_{i,j}^{(t)})$ to $\mathbf{x}_i^{(t)}$ and user $j(>i)$ subtracts $\mathrm{PRG}(a_{i,j}^{(t)})$ from $\mathbf{x}_j^{(t)}$.

% In the buffered asynchronous FL, however, the cancellation of the pairwise random masks based on the key agreement protocol is not guaranteed due to the mismatch in staleness between users. Specifically, at round $t$, user $i\in\mathcal{S}^{(t)}$ sends the masked model $\mathbf{y}_i^{(t;t_i)}$ to the server that is given by
% \begin{align} \small
%     \mathbf{y}_i^{(t;t_i)} &= {\Delta}^{(t;t_i)}_i + \mathrm{PRG}\left(b_i^{(t_i)}\right) \notag \\
%     &+\sum_{j: i<j} \mathrm{PRG}\left(a^{(t_i)}_{i, j}\right)-\sum_{j: i>j} \mathrm{PRG}\left(a^{(t_i)}_{j, i}\right),
% \end{align}
% where ${\Delta}^{(t;t_i)}_i$ is the local update of user $i$.
% When $t_i \neq t_j$, the pairwise random vectors in $\mathbf{y}_i^{(t;t_i)}$ and $\mathbf{y}_j^{(t;t_j)}$ are not canceled out as $a^{(t_i)}_{i, j} \neq a^{(t_j)}_{i, j}$.
% We note that the identity of the staleness of each user is not known a priori, hence each pair of users cannot use the same pairwise random-seed.

% \subsection{The \scheme Protocol in the Buffered Asynchronous FL}
% \label{subsec:proposed-async}

% To address the challenge of asynchrony, we generalize \scheme to the buffered asynchronous secure aggregation.
% Our key intuition is to encode the local masks in a way that the server can recover the aggregate of masks from the encoded masks via a one-shot computation even though the masks are generated in different training rounds.

% The generalized \scheme protocol also consists of three phases with three design parameters $D, T, U$ which are the same as the \scheme in the synchronous FL.
% The detailed steps of the generalized \scheme protocol is presented in the Appendix \ref{app:sub:async-lightsecagg}.

% \noindent{\bf Offline encoding and sharing of local masks.} 
% % Similar to the \scheme in the synchronous FL, user $i$ generates the random mask $\mathbf{z}_i^{(t_i)}$ and additional $T$ random masks denoted by $[\mathbf n^{(t_i)}_i]_{U-T+1}, \cdots, [\mathbf n^{(t_i)}_i]_{U}$. 
% User $i$ generates and sends the encoded masks $[\widetilde{\mathbf z}^{(t_i)}_i]_j$ to
% user $j\in[N]$ where $[\widetilde{\mathbf z}^{(t_i)}_i]_j$ is given in the same way in \eqref{eq:def_z_tilde} except for including local round index $t_i$.

% \noindent{\bf Masking and uploading of local updates.}

% \noindent{\bf One-shot aggregate-update recovery and global model update.}

==> MLSys/app_system.tex <==
\label{app:system}

\begin{figure}[h!]
% \captionsetup[subfigure]{justification=centering}
\centering
    % \subfigure[Aggregation Only]{\label{fig:pipeline_Aggr}
    % \includegraphics[width=.26\textwidth]{figures/Pipeline_AggrOnly.eps}
    % }
    \subfigure[ Non-overlapped ]{\label{fig:pipeline_NonOverlap}
    % \subfigure[Aggregation $+$ Training \newline (Non-overlapped)]{\label{fig:pipeline_NonOverlap}
    \includegraphics[width=.47\textwidth]{figures/Pipeline_NonOverlap.eps}
    }
    % \subfigure[Aggregation $+$ Training \newline (Overlapped)]{\label{fig:pipeline_Overlap}
    \subfigure[ Overlapped ]{\label{fig:pipeline_Overlap}
    \includegraphics[width=.47\textwidth]{figures/Pipeline_Overlap.eps}
    }
    \vspace{-4mm}
\caption{The timing diagram of the overlapped implementation in \scheme and \googlep \cite{bell2020secure} for a single FL training round to train MobileNetV3 \cite{howard2019searching} with CIFAR-100 dataset \cite{krizhevsky2009learning}. \google \cite{bonawitz2017practical} is not included as it takes much longer than other two protocols. }
\label{fig:pipeline}
\vspace{-3mm}
\end{figure}


